LEVER: Learning to Verify Language-to-Code Generation with Execution

The advent of large language models trained on code (code LLMs) has led to significant progress in language-to-code generation. State-of-the-art approaches in this area combine LLM decoding with sample pruning and reranking using test cases or heuristics based on the execution results. However, it is challenging to obtain test cases for many real-world language-to-code applications, and heuristics cannot well capture the semantic features of the execution results, such as data type and value range, which often indicates the correctness of the program. In this work, we propose LEVER, a simple approach to improve language-to-code generation by learning to verify the generated programs with their execution results. Specifically, we train verifiers to determine whether a program sampled from the LLMs is correct or not based on the natural language input, the program itself and its execution results. The sampled programs are reranked by combining the verification score with the LLM generation probability, and marginalizing over programs with the same execution results. On four datasets across the domains of table QA, math QA and basic Python programming, LEVER consistently improves over the base code LLMs(4.6% to 10.9% with code-davinci-002) and achieves new state-of-the-art results on all of them.

==> comments.tex <==
\an{
NL2Code is a set of important tasks --> 
    \begin{itemize}
        \item LLMs achieve good performance on such tasks with few-shot learning
        \item but it is hard to further improve their performance though finetuning because of the cost and accessibility
        \item How to improve (a black-box) LLM when more in-domain data is available 
    \end{itemize}
Key observation: when top-1 prediction is not right, the correct program can sometimes be found in its top k predictions, which suggests that LLMs may benefit from reranking --> \\
Idea: Reranking for NL2Code tasks -->
\begin{itemize}
    \item Programs can have very similar surface form but very different semantics, which is difficult to capture
    \item Denotation of programs from execution exposes the semantics of the programs, making it easier to distinguish different programs 
\end{itemize}
Thus we propose execution-augmented reranking.
Some other things I thought of:
\begin{itemize}
    \item Maybe we can also relate to domain adaptation?
\end{itemize}
}
\an{The motivation for using a separate model, few-shot learning has good recall but the accuracy is still }
\an{Ves: maybe discuss the difficulty of reranking and generation: reranking is probably easier, especially when we have execution. Discriminative reranking can be complement of generation from large models as it has access to richer information.}
\an{Scott: the key to make reranking work is what extra information we have, if execution is the key, we should talk more about the execution.}
\an{Sida: smth-augmented also doesn't sound exciting}
\an{Our method is a neural-symbolic-neural process}

==> tabs/codex_results_spider_wtq_wide.tex <==
\begin{table*}[]
    \centering
    \small
    \begin{tabular}{llllllllll}
        \toprule
        \multicolumn{2}{c}{\textbf{Spider}} &  & \multicolumn{3}{c}{\textbf{WTQ}} &  & \multicolumn{3}{c}{\textbf{GSM}} \\ 
                                \cline{1-2} \cline{4-6} \cline{8-10} 
        Methods            & Dev                    &  & Methods     & Dev      & Test          &  & Methods     & Dev      & Test    \\\midrule
        \multicolumn{10}{c}{\textit{Previous Work with Finetuning}} \\
        T5-3B \citep{xie2022unifiedskg}  & 71.8           &  & TaPEX \citep{liu2021tapex}       & 60.4 & 59.1   &  & SS \citep{ni2022learning}       & 20.7 & 19.5 \\
        Picard \citep{scholak2021picard} & 75.5                  &  & TaCube \citep{zhou2022tacube}    & 61.1 & 61.3   &  & SC \citep{welleck2022generating} & - & 24.2 \\
        RASAT \citep{qi2022rasat} & 80.5                  &  & OmniTab \citep{jiang2022omnitab} & -    & 63.3   &  & Diverse \citep{li2022advance} & - & 83.2 \\\midrule
        \multicolumn{10}{c}{\textit{Previous Work without Finetuning (all based on code-davinci-002)}} \\
        \citet{rajkumar2022evaluating}   & 67.0           &  & QA \citep{cheng2022binding}  & 50.5 & 48.7   &  & PAL \citep{gao2022pal} & - & 72.0 \\
                                         &                &  & SQL \citep{cheng2022binding}     & 60.2 & 61.1   &  & SC \citep{wang2022self} & - & 78.0 \\
                                         &                &  & Binder \citep{cheng2022binding}  & 65.0 & 64.6   &  & PoT-SC \citep{chen2022program} & - & 80.0 \\\midrule
        \multicolumn{10}{c}{\textit{This Work Using codex-davinci-002}} \\
        Greedy             & 75.3                   &  & Greedy      & 49.6             & 53.0             &  & Greedy      & 68.1     & 67.2    \\
        \oursf             & 81.9$_{0.1}$        &  & \oursf      & 64.6$_{0.2}$  & 65.8$_{0.2}$  &  & \oursf      & 84.1$_{0.2}$    & 84.5$_{\ph}$    \\
        % Oracle             & 92.9                   &  & Oracle      & 74.4     & 77.5          &  & Oracle      & 98.4     & 97.9    \\
        \bottomrule
    \end{tabular}
    
    % \begin{tabular}{lllllll}
    %     \toprule
    %     \multicolumn{3}{c}{\textbf{WTQ}} &  & \multicolumn{3}{c}{\textbf{GSM}} \\ 
    %                             \cline{1-3} \cline{5-7} 
    %     Methods     & Dev      & Test          &  & Methods     & Dev      & Test    \\\midrule
    %     \multicolumn{7}{c}{\textit{Previous Work with Finetuning}} \\
    %     TaPEX \citep{liu2021tapex}       & 60.4 & 59.1   &  & SS \citep{ni2022learning}       & 20.7 & 19.5 \\
    %     TaCube \citep{zhou2022tacube}    & 61.1 & 61.3   &  & SC \citep{welleck2022generating} & - & 24.2 \\
    %     OmniTab \citep{jiang2022omnitab} & -    & 63.3   &  & Diverse \citep{li2022advance} & - & 83.2 \\\midrule
    %     \multicolumn{7}{c}{\textit{Previous Work without Finetuning (all based on code-davinci-002)}} \\
    %     QA \citep{cheng2022binding}  & 50.5 & 48.7   &  & PAL \citep{gao2022pal} & - & 72.0 \\
    %     SQL \citep{cheng2022binding}     & 60.2 & 61.1   &  & SC \citep{wang2022self} & - & 78.0 \\
    %     Binder \citep{cheng2022binding}  & 65.0 & 64.6   &  & PoT-SC \citep{chen2022program} & - & 80.0 \\\midrule
    %     \multicolumn{7}{c}{\textit{This Work Using codex-davinci-002}} \\
    %     Greedy      & 49.6             & 53.0             &  & Greedy      & 68.1     & 67.2    \\
    %     \oursf      & 64.6$_{\pm0.2}$  & 65.8$_{\pm0.2}$  &  & \oursf      & 84.1$_{\pm0.2}$    & 84.5$_{\ph}$    \\
    %     % Oracle             & 92.9                   &  & Oracle      & 74.4     & 77.5          &  & Oracle      & 98.4     & 97.9    \\
    %     \bottomrule
    % \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}

==> tabs/few_shot_settings.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\small
\centering
\begin{tabular}{l|c|ccc}
\toprule
\multirow{2}{*}{\textbf{Datasets}} & \multirow{2}{*}{\textbf{Phase}} & \textbf{Codex} & \textbf{InCoder} & \textbf{CodeGen} \\
                                   &                                 & (T=0.6)        & (T=0.8)             & (T=0.8)              \\\midrule
Spider                             & Train                           & 20             & 50                  & 50                   \\
                                   & Test                            & 50             & 100                 & 100                  \\\hline
\multirow{2}{*}{SQUALL}            & Train                           & 50             & -                   & -                    \\
                                   & Test                            & 50             & -                   & -                    \\\hline
\multirow{2}{*}{GSM}               & Train                           & 50             & 50                  & 50                   \\
                                   & Test                            & 100             & 100                 & 100                  \\\hline
\multirow{2}{*}{MBPP}              & Train                           & 100            & -                   & -                    \\
                                   & Test                            & 100            & -                   & -                    \\\bottomrule
\end{tabular}
\caption{Detailed sampling budget and temperature for different code LLMs on all four tasks. ``Phrase'' refers to the train/test time settings.}
\label{tab:few-shot-settings}
\end{table}

==> tabs/main_codex_result.tex <==
\begin{table}
\small
\centering
\begin{tabular}{lllll}
\toprule
\textbf{Methods} & \textbf{Spider} & \textbf{WTQ} & \textbf{GSM} & \textbf{MBPP}\\
\midrule
\multicolumn{2}{l}{\textit{Previous SoTA:}} \\
\quad Finetuned     & $80.5^a$ & $63.3^b$ & $83.2^c$ & \quad-\footnotemark \\
\quad Few-shot      & $67.0^d$ & $64.6^e$ & $80.0^f$ & $66.9^g$ \\\midrule
\multicolumn{3}{l}{\textit{Baselines}:} \\
\quad Greedy        & 75.3 & 53.0 & 67.2 & 62.0 \\
\quad ML            & 75.0 & 53.0 & 49.8 & 59.0 \\
\quad ML + EP       & 77.3 & 54.9 & 72.6 & 60.2 \\
\quad Voting        & 78.8 & 56.0 & 79.2 & 66.2 \\\hdashline
\oursf              &\textbf{81.9}$_{\pm0.1}$   & \textbf{65.8}$_{\pm0.2}$
                    &\textbf{84.1}$_{\ph}$      & \textbf{68.9}$_{\pm0.4}$ \\
\quad - exec.       & 79.0 & 60.5 & 83.0 & 66.1 \\\midrule
\textit{Oracle}     & 92.9 & 77.5 & 97.9 & 91.4 \\
\bottomrule
\end{tabular}

% \begin{tabular}{lcclccclccclcc}
% \toprule
% \multicolumn{2}{c}{\textbf{Spider}} &  & \multicolumn{3}{c}{\textbf{WTQ}} &  & \multicolumn{3}{c}{\textbf{GSM}} &  & \multicolumn{3}{c}{\textbf{MBPP}} \\ \cline{1-2} \cline{4-6} \cline{8-10} \cline{12-14} 
% Methods            & Dev            &  & Methods     & Dev      & Test    &  & Methods     & Dev      & Test    &  & Methods     & Dev      & Test     \\\midrule
% \multicolumn{14}{c}{\textit{Previous Work - with Finetuning}} \\\midrule
% % \citet{qi2022rasat} & 80.5 & & \citet{jiang2022omnitab} & & & & \citet{li2022advance} & & & & \citet{zhang2022coder} \\
% \multicolumn{14}{c}{\textit{Previous Work - without Finetuning}} \\\midrule
% \multicolumn{14}{c}{\textit{Code-davinci-002}} \\\midrule
% Greedy             & 75.3           &  & Greedy      & 49.6     & 53.0    &  & Greedy      & 68.1     & 67.2    &  & Greedy      & 61.1     & 62.0     \\
% Ours               & 82.0           &  & Ours        & 64.8     & 66.1    &  & Ours        & 84.1     & 84.5    &  & Ours        & 76.1     & 68.5     \\\midrule
% Oracle             & 92.9           &  & Oracle      & 74.4     & 77.5    &  & Oracle      & 98.4     & 97.9    &  & Oracle      & 91.1     & 91.4     \\\bottomrule
% \end{tabular}

\caption{Main results with the \texttt{code-davinci-002} model on the test sets (dev set used for Spider). ``Oracle'' denotes the upper-bound of the reranking method, details on baselines can be found in \autoref{sec:baseline-details}.
Previous SoTA numbers are taken from $^a$: RASAT \citep{qi2022rasat}; $^b$: OmniTab \citep{jiang2022omnitab}; $^c$: DiVerSE \citep{li2022advance}; $^d$: \citet{rajkumar2022evaluating}; $^e$: BINDER \citep{cheng2022binding}; $^f$: PoT \citep{chen2022program}; $^g$: Reviewer \citep{zhang2022coder}.
% \victoria{For the SOTA numbers shown here, denote which baseline is supervised and which one is few-shot.}
}
\label{tab:main-codex-result}
\end{table}
\footnotetext{Though we can not find finetuned execution accuracy (\ie pass@1) performance, as a reference, \citet{austin2021program} reported their pass@80 and acc@80 to be ~62\% and ~14\% for the finetuned 137B model.}
